PowerTransformer: Unsupervised Controllable Revision for Biased Language Correction

Unconscious biases continue to be prevalent in modern text and media, calling for algorithms that can assist writers with bias correction. For example, a female character in a story is often portrayed as passive and powerless ("She daydreams about being a doctor") while a man is portrayed as more proactive and powerful ("He pursues his dream of being a doctor"). We formulate *Controllable Debiasing*, a new revision task that aims to rewrite a given text to correct the implicit and potentially undesirable bias in character portrayals. We then introduce PowerTransformer as an approach that debiases text through the lens of connotation frames (Sap et al., 2017), which encode pragmatic knowledge of implied power dynamics with respect to verb predicates. One key challenge of our task is the lack of parallel corpora. To address this challenge, we adopt an unsupervised approach using auxiliary supervision with related tasks such as paraphrasing and self-supervision based on a reconstruction loss, building on pretrained language models. Through comprehensive experiments based on automatic and human evaluations, we demonstrate that our approach outperforms ablations and existing methods from related tasks. Furthermore, we demonstrate the use of PowerTransformer as a step toward mitigating the well-documented gender bias in character portrayal in movie scripts.

==> 12-old-task-desc.tex <==
\maarteninline{really highlight the machine in the loop writing angle. Also, here we can re-introduce the connotation frames again in high-level.
And again, we should make it clear that to debias the portrayal sometimes we have to go beyond paraphrasing and change the denotational meaning.}
We define \taskname as a new formalization of the controllable rewriting task that aims to alter a the connoted agency of the characters described in a sentence.


Using text classification terminology from \citet{card.2018.proportions}, we focus on changing the connotations of text that are evoked in the reader (\textit{extrinsic}), in contrast to most previous work which alters the characteristics that led to the creation of the text \cite[\textit{intrinsic}; e.g., author gender, sentiment of review;][]{Prabhumoye2018-kj,?}.
With intrinsic style rewriting, the distinction between the style and meaning is often ill-defined, causing models to drastically change the factual meaning of sentence (e.g., a review about an  Italian restaurant rewritten to be about a Mexican restaurant).
Here, we use the distinction between connoted and denoted meaning to guide our rewriting task, so we can aim to alter only the connoted meaning.
% can focus on rewriting the connoted meaning while aiming to preserve as much of the holistic events described.


Focusing on the implied meanings in text, \taskname can help in editing out unconscious social biases in text (e.g., that women experience change rather than drive it; Figure \ref{fig:introFig}).
Text is known to reflect social and societal inequality \cite[e.g., power dynamics between genders][]{lakoff1973language}, and (unconsciously biased) implied meaning can be used to exacerbate this inequality \cite{Fiske1993controlling,sap2020socialbiasframes}.
\taskname could therefore be useful as a machine-in-the-loop writing system \cite[e.g., ][Textio]{clark2018creative}\footnote{\url{https://textio.com/}}, to help authors portray characters more equitably by providing phrasings with alternate connoted meanings.


% \maarteninline{Maybe we can contrast what ``style'' means using Dallas' intrinsic vs. extrinsic text labels definitions \cite{card.2018.proportions}, and merge them with denotational vs. connotational meaning.
% A lot of style transfer has focused on intrinsic properties of text (e.g., the political leaning or gender of the author). Changing those is arguably just pushing the limits of what NLP can do but not of any real use in society (but like... we won't actually say that).

% Extrinsic labels are ones that are more related to the reaction that is evoked from text (e.g., agency? Maybe politeness but I'm not sure about that one.).
% This is what our task is about: changing the text so that it changes the ``reaction'' that is evoked in the reader, without necessarily changing its content / intrinsic properties.
% And that allow for social impact because we know that some of the connotations are really biased.
% }


% % \subsection{\taskname}
% \hannahinline{Need to highlight everything that makes this unique compared to traditional style transfer!  And the fact that this task is a novel use of re-writing for connotation, possibly highlighting the far-reaching downstream applications of this.}


==> 13-old.methods.tex <==

\hannah{TODO: I put the ablations, baselines, set-up in the experimental details already, so we can remove from this section. we need to rewrite this section, so that it's just focusing on the Joint+Static model in a top-down fashion.  we need to add a modeling figure and equations.}

\maarteninline{Notes on restructuring:
The current setup follow the way that we built up our model, but isn't necessarily the way that NLP papers usually present models. Also note, people don't usually discuss results in the modelling section, and often times we separate the empirical details/hyperparams from the high-level modelling ideas.
We should try to always make the most important thing the first thing we talk about: our final model!
Note, while you're writing, pretend like there's a model overview figure that you can refer back to!
See proposed high-level structure below.}

\maarteninline{Introduce the \modelname's high-level design, saying it's an encoder-decoder that relies on three components that are shown in Figure 2 (to be made LOL).
Also high-level say that we use two sources of data for these two components, described in data sections
}
Given an input sentence with unconscious bias, we would like to rewrite it preserving its original context while changing its agency level. We first denoise the input sentence which makes it agency neutral as described in \ref{sec:denoise}. We set up an encoder-decoder model that takes the input sentence after denoising and the desired agency category then outputs the rewritten sentences.

\subsection{Encoder-decoder with style}\maarten{need better heading}
\maarteninline{Describe the encoder-decoder general setup, including the desired attribute token. Maybe we can use Figure 2 to describe the exact ordering of variables.}
We load OpenAI GPT LM model as our pre-trained model and add a few special tokens for agency classes. 
\begin{center}
\begin{tabular}{ c c }
 CLS & classification token for target agency \\
 POS & positive agency \\
 EQUAL & equal agency \\
 NEG & negative agency 
\end{tabular}
\end{center}
For a denoised sentence, we set up the training instance as 
\begin{verbatim}
SentenceDenoised CLS POS Sentence
\end{verbatim}
if the desired agency is positive and evaluate the CrossEntropyLoss on Sentence. At generation time, we give 
\begin{verbatim}
SentenceDenoised CLS POS
\end{verbatim}
and the model is supposed to add positive agency to the devnoised sentence.

\subsection{Learning to denoise with style}\maarten{Need better heading}
\label{sec:denoise}
\maarteninline{Describe the denoising setup, specifically how we delete verbs, etc.}
\cite{sap2017connotation} gives an agency lexicon of verbs. We classify the sentences by the max number of verbs in the agency category. For example, if a sentence has two positive agency verbs and one negative agency verb, the sentence will be classified as positive agency. During training time, we deleted sentences with 4 or more agency verbs to avoid confusion. Then, any verb in the sentence agency category is deleted and replaced by a special token VERB to indicate there used to be verb in the input sentence.

\subsection{Learning to paraphrase with style}\maarten{Need better heading}
\maarteninline{Describe the paraphrase setup, and explain how we }
For paraphrase corpus, we denoise the original sentence, set the target agency to be the agency of the paraphrase sentence and put the paraphrase sentence as the target generation, so the input becomes
\begin{verbatim}
SentenceDenoised CLS POS Paraphrase
\end{verbatim}
if the paraphrase sentence is positive agency.


\subsection{Baselines}
\maarteninline{Explain the baselines that we use. Try to frame it as ``things that we changed/removed from the main model'' and make sure to have a high-level intuition /motivation for each of the baselines (e.g., ``to examine the effect of logit rescaling, we have a baseline without it'')}

\paragraph{baseline 1}
We have considered not doing the denoising step and just add logits at generation time. The training instance looks similar to the one mentioned in Section 3.1 except we do not denoise the original sentence.
\begin{verbatim}
OriginalSentence CLS POS Sentence
\end{verbatim}
At generation time, we set up the input as 
\begin{verbatim}
OriginalSentence CLS POS
\end{verbatim}
and boost the logits for verbs in the desired agency. Without denoising, the model would need to counteract the original agency, thus we do a scaling instead of adding logits with $\beta = 1.5$.

\paragraph{Joint-NoBoost}
We also examine the effect of adding logits by inspecting the encoder-decoder setup without boosting logits, which is our Joint-NoBoost model.

\paragraph{baseline 3}
Since boosting the logits helps greatly with generation at the desired agency, we wonder if supplying the verbs themselves would produce a similar result. Thus we explore another setting of the encoder-decoder model. At training time, we append the verbs we deleted instead of the agency category after the denoised sentence and we do the same for both ROC story and paraphrase data. The training instance becomes 
\begin{verbatim}
SentenceDenoised DeletedVerbs TargetSentence
\end{verbatim}
For ROC stories, the TargetSentence is the sentence itself, and with paraphrase data, we set the TargetSentence to be the paraphrase sentence.
At generation time, since we do not know what verbs are supposed to be inserted, we supply a similar word in the agency we want to generate. The input becomes
\begin{verbatim}
SentenceDenoised SimilarVerb
\end{verbatim}
% need to add citation on the noise fraction
We determine the word similarity by calculating the cosine similarity between two words in their glove 300d vector and choose the word with the smallest cosine similarity. Since the lexica contains a rather smaller verb set(2146 in total), occasionally words irrelevant to the sentence context are given to the model, which does not help with the generation.
Giving the exact deleted verbs often leads to the modeling simply inserting the given verbs into the deleted location. Inspired by CITATION, we define a percentage fraction $\alpha$, and for $\alpha$ per cent of the input, instead of supplying the deleted verb, we instead supply a similar verb in the same agency category using cosine similarity. We found $\alpha = 0.1$ for ablation study.


\subsection{Experimental Details}
\hannah{rewrite so that there's a dedicated ``logits boosting'' subsection that's a bit more emphasized}
In order to further force generation of desired agency, we add some logits on the vocab at generation time of each token. For each verb in the desired agency, set its logits addition to 1 with all tenses and for other words 0. The logits are than scaled by a constant $\beta$ to control the degree of agency generation. We find $\beta=5$ a decent value that directs the generation and does not lead to too much repetition issues.




\section{Previous modelling section}


% TODO: perplexity and bigram repetition
% Also use add logits for this implementation
% And this data is on model trained on paraphrase, and need to train the model on mix and look at the stats

\subsection{Learning the logistic scaling factor}
Inspired by AffectLM architectural, we added a learnable weight on top of the DelRet model and the resulting logits becomes
\[Logit = LM logits +  W(c)\]
where LM logits are the outputs from the DelRet model, W is a $C \wedge V$ matrix with C denoting the number of agency categories. Similar to \logitRescaling, we are adding some agency specific logits on top of the language model and we are allowing the model to learn how much logits to add to each word during training. At generation time, we take the W from training and apply it to the DelRet model 
\[Logit = LM logits + \beta W(c)\]
with $\beta$ controling how much influence we would like to add to the model.
\subsubsection{Cumulative agency category}
We set c for each word to the number of words in one agency category up to this word and we do this for each agency category. We tried to train the model in both language model setting and delete retrieve setting and take W out and add to the best-performed delRet model. It seems that the model learns to counteract with the supplied agency, since negative $\beta$ makes it more likely to generate verbs in the destination agency.
\subsubsection{Word-level agency Category}
We set c to 1 only for the word with agency label. Since we have a rather small vocab for agency words, on average a sentence will have one or two words with agency level. Thus the model does not learn a lot from the addition information.
\subsubsection{Sentence level agency category}
We set c to the number of words in each category in the entire sentence for each word in the sentence. This forces the model to learn the correlation between agency and words.


\subsection{Datasets}



%% DATA STATS:
% details about paraphrase dataset, details about ROC dataset
% table with number of train/dev/test examples
% avg # tokens per example (split by train/dev/test maybe?)

\maarten{Do we like this section here?}
We use individual sentences from ROC stories as our primary resource for re-writing.  Because we do not have parallel story data, at training time, we additionally leverage noisy examples of parallel sentences with different connotations, which we construct from a paraphrase corpus.

\paragraph{Roc Story Data}
%all the details...


\paragraph{Paraphrase Data}
%all the details...


==> old-intros.tex <==
Rewriting text with a specified style of framing, i.e., \textit{controllable rewriting}, alters the reader's interpretation of the events and people described in the text.
Since most human written text reflects societal biases (e.g., stereotypes, gender bias), controllable rewriting can help with de-biasing these texts by, for example, reducing the gender bias in how agentic and decisive characters are described. 
For example, rewriting the story sentence ``Agatha saw the office workers'' in a story


Rewriting text with a specified style or framing can alter the way the text is read and the conclusions that are drawn from it (e.g., character portrayal).

Successfully doing so requires preserving the denotational meaning of text while altering its connotative meaning. This is hard because we don't have parallel data. And prior work (e.g., in sentiment) has show that factual meaning is often altered because they used "domains" as definitions etc.



\maarten{Story version with controllable rewriting angle}
The key challenge to successfully paraphrasing text with a purpose is overcoming the absence of parallel data to train on, preventing the use of traditional encoder-decoder systems.
Additionally, such systems often struggle to preserve the factual meaning of the input when paraphrasing to a target style, as shown by previous work \cite{previousWork}.

\maarten{Story version more focused on the portrayal angle}
When stories are written, authors portray characters through actions and their implied connotations \cite{something}.
\maarten{Replace with actual example from Fig 1}
For example, in Figure \ref{fig:introFig}, the sentence ``\textit{Adriana supervised her office employees}'' implies that Adriana has more agency than when she simply ``\textit{sees the office workers}.''
These portrayal differences are often aligned with existing societal stereotypes\cite[e.g., women are frequently portrayed with less agency than men in media;][]{sap2017connotation,field2019contextual}.
